Storage Participation in Electricity Markets: Time Discretization through Robust Optimization

Electricity storage is used for intertemporal price arbitrage and for ancillary services that balance unforeseen supply and demand fluctuations via frequency regulation. We present an optimization model that computes bids for both arbitrage and frequency regulation and ensures that storage operators can honor their market commitments at all times for all fluctuation signals in an uncertainty set inspired by market rules. This requirement, initially expressed by an infinite number of nonconvex functional constraints, is shown to be equivalent to a finite number of deterministic constraints. The resulting formulation is a mixed-integer bilinear program that admits mixed-integer linear relaxations and restrictions. Empirical tests on European electricity markets show a negligible optimality gap between the relaxation and the restriction. The model can account for intraday trading and, with a solution time of under 5 seconds, may serve as a building block for more complex trading strategies. Such strategies become necessary as battery capacity exceeds the demand for ancillary services. In a backtest from 1 July 2020 through 30 June 2024 joint market participation more than doubles profits and almost halves energy output compared to no FCR participation.

==> 8_countries.tex <==
\section{Multi-country comparison} \label{sec:country}
\begin{table}[H]
\tiny
\centering
\begin{tabular}{l|lllll}
    Country & AT & BE & CH & DE & NL \\
    No FCR Mean profit/day (\EUR) & \phantom{00}5.599 & \phantom{00}7.175 & \phantom{00}3.324 & \phantom{00}6.971 & \phantom{00}7.948 \\
    Restrict Mean profit/day (\EUR) & \phantom{00}6.818 & \phantom{00}7.986 & \phantom{00}5.417 & \phantom{00}7.809 & \phantom{00}8.700 \\
    Restrict Mean FCR profit/day (\EUR) & \phantom{00}2.782 & \phantom{00}2.047 & \phantom{00}3.630 & \phantom{00}2.194 & \phantom{00}1.925 \\
    No FCR Mean throughput/day (kWh) & 142.582 & 161.586 & 116.258 & 148.105 & 157.982 \\
    Restrict Mean throughput/day (kWh) & \phantom{0}90.458 & 118.327 & \phantom{0}58.560 & 103.746 & 117.620 \\
\end{tabular}
\caption{Country comparison results summary}
\label{tab:res_country}
\end{table}

We extend the results from \Cref{sec:backtesting} to additional energy markets using data from countries participating in the Regelleistung.net data archive across the experimental horizon, enabling comparisons across Austrian, Belgian, German, and Dutch energy markets in addition to the French market. In the following experiments we continue to use the French RTE frequency data to generate the frequency regulation signal as all countries energy markets operate within the same synchronous market (TODO: cite).

From these experiments we observe four main market context groupings: Switzerland, Austria and France, Germany and Belgium, and the Netherlands. Overall the Swiss market provides the lowest total profit incentives for a battery storage operator in both day-ahead and joint market participation. However, the smaller arbitrage opportunities also cause the Swiss market to contain the highest impact of joint participation with 63\% profit improvement and 64\% reduction in throughput over just day-ahead participation. The Austrian and French markets both contain comparatively low arbitrage opportunities in day-ahead markets compared to Belgian, German, and Dutch markets and a comparatively high impact of joint market participation with profit improvements of 21.8\% and 21.7\% respectively and a throughput decrease of 36.6\% and 34.9\% respectively. In contrast, the Belgian and German markets contain more profitable arbitrage opportunities but a smaller impact of joint market participation with profit improvements of 11.3\% and 12.0\% respectively and a throughput decrease of 26.8\% and 30.0\% respectively. Finally, the Dutch market contains the most profitable arbitrage opportunities in our data. This higher profitability of arbitrage also leads to the lower impact of joint market participation as the incentives skew towards continuing to offer larger amounts of power on the day ahead market with a mean profit improvement of 9.5\% and throughput reduction of 25.5\%.

Despite regional differences, across all cases joint market participation makes energy storage more attractive with consistent increases in profit and decreases in throughput. Additionally, we observed the magnitude of beneficial effects of joint market participation to be inversely correlated to the existing day-ahead market arbitrage opportunities, thus providing the combined impact of encouraging battery deployment in places where batteries are already being used and helping to start deployment where they have not been historically developed.

